Towards device-independent information processing on general quantum networks

The violation of certain Bell inequalities allows for device-independent information processing secure against non-signalling eavesdroppers. However, this only holds for the Bell network, in which two or more agents perform local measurements on a single shared source of entanglement. To overcome the practical constraint that entangled systems can only be transmitted over relatively short distances, large-scale multi-source networks have been employed. Do there exist analogues of Bell inequalities for such networks, whose violation is a resource for device-independence? In this paper, the violation of recently derived polynomial Bell inequalities will be shown to allow for device-independence on multi-source networks, secure against non-signalling eavesdroppers.

==> library.tex <==
@article{lee2016deriving,
  title={Deriving Grover's lower bound from simple physical principles},
  author={Lee, Ciar{\'a}n M and Selby, John H},
  journal={New Journal of Physics},
  volume={18},
  issue={9},
  number={093047},
  year={2016},
  publisher={IOP Publishing}
}

@article{yin2017satelite,
title={Satellite-based entanglement distribution over 1200 kilometers},
author={Yin, Juan and et al.},
journal={Science, Vol. 356, Issue 6343, pp. 1140-1144},
year={2017}
}

@article{masanes2011,
  title={Secure device-independent quantum key distribution with causally independent measurement devices},
  author={Masanes, Llu\'{i}s and Pironio, Stefano and Ac{\'\i}n, Antonio},
  journal={Nature Communications},
  volume={2},
  number={238},
  year={2011},
  publisher={Nature} 
}

@article{gallegoseq,
  title={Nonlocality in sequential correlation scenarios},
  author={Gallego, Rodrigo and W\"{u}rflinger, Lars E. and Chaves, Rafael and Ac\'{i}n, Antonio and  Navascu\'{e}s, Miguel},
  journal={New Journal of Physics},
  volume={16},
  number={033037},
  year={2014},
  publisher={IOP Publishing} 
}

@article{curchod2017,
  title={Unbounded randomness certification using sequences of measurements},
  author={Curchod, F. and Johansson, M. and Augusiak, R. and Hoban, M. J. and Wittek, P. and Ac\'{i}n, A.},
  journal={Phys. Rev. A},
  volume={95},
  number={020102(R)},
  year={2017},
  publisher={APS} 
}

@article{seri2017quantum,
  title={Quantum Correlations between Single Telecom Photons and a Multimode On-Demand Solid-State Quantum Memory},
  author={Seri, Alessandro and Lenhard, Andreas and Riel{\"a}nder, Daniel and G{\"u}ndo{\u{g}}an, Mustafa and Ledingham, Patrick M and Mazzera, Margherita and de Riedmatten, Hugues},
  journal={Physical Review X},
  volume={7},
  issue={2},
  number={021028},
  year={2017},
  publisher={APS}
}

@article{nunn2017solid,
  title={A Solid Footing for a Quantum Repeater},
  author={Nunn, Joshua},
  journal={Physics},
  volume={10},
  pages={55},
  year={2017},
  publisher={APS}
}

@article{valivarthi2016quantum,
  title={Quantum teleportation across a metropolitan fibre network},
  author={Valivarthi, Raju and Zhou, Qiang and Aguilar, Gabriel H and Verma, Varun B and Marsili, Francesco and Shaw, Matthew D and Nam, Sae Woo and Oblak, Daniel and Tittel, Wolfgang and others},
  journal={Nature Photonics},
  volume={10},
  number={10},
  pages={676--680},
  year={2016},
  publisher={Nature Research}
} 

@article{sun2016quantum,
  title={Quantum teleportation with independent sources and prior entanglement distribution over a network},
  author={Sun, Qi-Chao and Mao, Ya-Li and Chen, Si-Jing and Zhang, Wei and Jiang, Yang-Fan and Zhang, Yan-Bao and Zhang, Wei-Jun and Miki, Shigehito and Yamashita, Taro and Terai, Hirotaka and others},
  journal={Nature Photonics},
  year={2016},
  publisher={Nature Research}
}

@book{van2014quantum,
  title={Quantum networking},
  author={Van Meter, Rodney},
  year={2014},
  publisher={John Wiley \& Sons}
}

@article{taherkhani2017resource,
  title={Resource-aware architecture for implementation of quantum aided Byzantine agreement on quantum repeater networks},
  author={Taherkhani, M Amin and Navi, Keivan and Van Meter, Rodney},
  journal={arXiv preprint arXiv:1701.04588},
  year={2017}
}

@article{satoh2012quantum,
  title={Quantum network coding for quantum repeaters},
  author={Satoh, Takahiko and Le Gall, Fran{\c{c}}ois and Imai, Hiroshi},
  journal={Physical Review A},
  volume={86},
  issue={3},
  number={032331},
  year={2012},
  publisher={APS}
}

@article{satoh2017network,
  title={The Network Impact of Hijacking a Quantum Repeater},
  author={Satoh, Takahiko and Nagayama, Shota and Van Meter, Rodney},
  journal={arXiv preprint arXiv:1701.04587},
  year={2017}
}

@article{anders2009computational,
  title={Computational power of correlations},
  author={Anders, Janet and Browne, Dan E},
  journal={Phys. Rev. Lett.},
  volume={102},
  issue={5},
  number={050502},
  year={2009},
  publisher={APS}
}

@article{rozpedek2017relaistic,
  title={Realistic parameter regimes for a single sequential quantum repeater},
  author={Rozpedek, Filip and Goodenough, Kenneth and Ribeiro, Jérémy and Kalb, Norbert and Vivoli, Valentina Caprara and Reiserer, Andreas and Hanson, Ronald and Wehner, Stephanie and Elkouss, David},
  journal={arXiv preprint arXiv:1705.00043},
  year={2017}
}

@article{goodenough2016assessing,
  title={Assessing the performance of quantum repeaters for all phase-insensitive Gaussian bosonic channels},
  author={Goodenough, Kenneth and Elkouss, David and Wehner, Stephanie},
  journal={New Journal of Physics},
  volume={18},
  issue={6},
  number={063005},
  year={2016},
  publisher={IOP Publishing}
}

@article{reiserer2016robust, 
  title={Robust quantum-network memory using decoherence-protected subspaces of nuclear spins},
  author={Reiserer, Andreas and Kalb, Norbert and Blok, Machiel S and van Bemmelen, Koen JM and Taminiau, Tim H and Hanson, Ronald and Twitchen, Daniel J and Markham, Matthew},
  journal={Physical Review X},
  volume={6},
  issue={2},
  number={021040},
  year={2016},
  publisher={APS}
}

@article{van2017multiplexed, 
  title={Multiplexed entanglement generation over quantum networks using multi-qubit nodes},
  author={van Dam, Suzanne B and Humphreys, Peter C and Rozpedek, Filip and Wehner, Stephanie and Hanson, Ronald},
  journal={arXiv preprint arXiv:1702.04885},
  year={2017}
}

@article{sangouard2011quantum, 
  title={Quantum repeaters based on atomic ensembles and linear optics},
  author={Sangouard, Nicolas and Simon, Christoph and De Riedmatten, Hugues and Gisin, Nicolas},
  journal={Reviews of Modern Physics},
  volume={83},
  number={1},
  pages={33},
  year={2011},
  publisher={APS}
}

@article{andreoli2017maximal,
  title={Maximal violation of n-locality inequalities in a star-shaped quantum network},
  author={Andreoli, Francesco and Carvacho, Gonzalo and Santodonato, Luca and Chaves, Rafael and Sciarrino, Fabio},
  journal={arXiv preprint arXiv:1702.08316},
  year={2017}
}

@article{Tavakoli2017correlations, 
  title={Correlations in star networks: from Bell inequalities to network inequalities},
  author={Tavakoli, Armin and Renou, Marc Olivier and Gisin, Nicolas and Brunner, Nicolas},
  journal={arXiv preprint arXiv:1702.03866},
  year={2017}
}

@article{andreoli2017experimental,
  title={Experimental bilocality violation without shared reference frames},
  author={Andreoli, Francesco and Carvacho, Gonzalo and Santodonato, Luca and Bentivegna, Marco and Chaves, Rafael and Sciarrino, Fabio},
  journal={arXiv preprint arXiv:1705.03309},
  year={2017}
}

@article{carvacho2017experimental, 
  title={Experimental violation of local causality in a quantum network},
  author={Carvacho, Gonzalo and Andreoli, Francesco and Santodonato, Luca and Bentivegna, Marco and Chaves, Rafael and Sciarrino, Fabio},
  journal={Nature Communications},
  issue={8},
  number={14775},
  year={2017},
  publisher={Nature Publishing Group}
}

@article{saunders2017experimental, 
  title={Experimental demonstration of nonbilocal quantum correlations},
  author={Saunders, Dylan J and Bennet, Adam J and Branciard, Cyril and Pryde, Geoff J},
  journal={Science Advances},
  volume={3},
  issue={4},
  number={e1602743},
  year={2017},
  publisher={American Association for the Advancement of Science}
}

@article{braunstein1990wringing,
  title={Wringing out better Bell inequalities},
  author={Braunstein, Samuel L and Caves, Carlton M},
  journal={Annals of Physics},
  volume={202},
  number={1},
  pages={22--56},
  year={1990},
  publisher={Elsevier}
}

@article{wehner2006tsirelson,
  title={Tsirelson bounds for generalized clauser-horne-shimony-holt inequalities},
  author={Wehner, Stephanie},
  journal={Physical Review A},
  volume={73},
  issue={2},
  number={022110},
  year={2006},
  publisher={APS}
}

@article{pironio2010random,
  title={Random numbers certified by Bell's theorem},
  author={Pironio, Stefano and Ac{\'\i}n, Antonio and Massar, Serge and de La Giroday, A Boyer and Matsukevich, Dzimitry N and Maunz, Peter and Olmschenk, Steven and Hayes, David and Luo, Le and Manning, T Andrew and others},
  journal={Nature},
  volume={464},
  issue={7291},
  pages={1021--1024},
  year={2010},
  publisher={Nature Publishing Group}
} 

@article{pironio2009device,
  title={Device-independent quantum key distribution secure against collective attacks},
  author={Pironio, Stefano and Ac\'{i}n, Antonio and Brunner, Nicolas and Gisin, Nicolas and Massar, Serge and Scarani, Valerio},
  journal={New Journal of Physics},
  volume={11},
  issue={4},
  number={045021},
  year={2009},
  publisher={IOP Publishing}
}

@article{hoban2011generalized,
  title={Stronger Quantum Correlations with Loophole-free Post-selection},
  author={Hoban, Matty J and Browne, Dan E},
  journal={Phys. Rev. Lett.},
  volume={107},
  number={120402},
  year={2011},
  publisher={APS}
}

@article{wallman2014nonlocality,
  title={Nonlocality in instantaneous quantum circuits},
  author={Wallman, Joel J and Adlam, Emily},
  journal={arXiv preprint arXiv:1412.4131},
  year={2014}
}

@article{acin2006bell, 
  title={From Bell's theorem to secure quantum key distribution},
  author={Ac\'{i}n, Antonio and Gisin, Nicolas and Masanes, Lluis},
  journal={Phys. Rev. Lett.},
  volume={97},
  issue={12},
  number={120405},
  year={2006},
  publisher={APS}
}

@BOOK{Pearl-09, 
 author={Judea Pearl},
 title={Causality: Models, Reasoning, and Inference},
 edition={2nd},
 publisher={Cambridge University Press},
 address={Cambridge},
 year={2009}
}

@BOOK{Spirtes-Glymour-01,
 author={Peter Spirtes and Clark Glymour and Richard Scheines},
 title={Causation, Prediction, and Search},
 edition={2nd},
 publisher={The MIT Press}, 
 address={Cambridge, MA}, 
 year={2001}
}

@article{brask2017bell,
  title={Bell scenarios with communication},
  author={Brask, Jonatan Bohr and Chaves, Rafael},
  journal={Journal of Physics A: Mathematical and Theoretical},
  year={2017},
  publisher={IOP Publishing}
}

@article{chaves2016causal,
  title={Causal hierarchy of multipartite Bell nonlocality},
  author={Chaves, Rafael and Cavalcanti, Daniel and Aolita, Leandro},
  journal={arXiv preprint arXiv:1607.07666},
  year={2016}
}

@article{fritz2012beyond,
  title={Beyond Bell's theorem: correlation scenarios},
  author={Fritz, Tobias},
  journal={New Journal of Physics},
  volume={14},
  issue={10},
  number={103001},
  year={2012},
  publisher={IOP Publishing}
}

@article{henson2014theory,
  title={Theory-independent limits on correlations from generalized Bayesian networks},
  author={Henson, Joe and Lal, Raymond and Pusey, Matthew F},
  journal={New Journal of Physics},
  volume={16},
  issue={11},
  number={113043},
  year={2014},
  publisher={IOP Publishing}
}

@article{wood2015lesson,
  title={The lesson of causal discovery algorithms for quantum correlations: Causal explanations of Bell-inequality violations require fine-tuning},
  author={Wood, Christopher J and Spekkens, Robert W},
  journal={New Journal of Physics},
  volume={17},
  issue={3},
  number={033002},
  year={2015},
  publisher={IOP Publishing}
}

@article{chaves2015unifying,
  title={Unifying framework for relaxations of the causal assumptions in Bell's theorem},
  author={Chaves, Rafael and Kueng, Richard and Brask, Jonatan Bohr and Gross, David},
  journal={Phys. Rev. Lett.},
  volume={114},
  issue={14}, 
  number={140403},
  year={2015},
  publisher={APS}
}

@article{barrett2005no,
  title={No signaling and quantum key distribution},
  author={Barrett, Jonathan and Hardy, Lucien and Kent, Adrian},
  journal={Phys. Rev. Lett.},
  volume={95},
  issue={1},
  number={010503},
  year={2005},
  publisher={APS}
}

@article{barrett2006maximally,
  title={Maximally nonlocal and monogamous quantum correlations},
  author={Barrett, Jonathan and Kent, Adrian and Pironio, Stefano},
  journal={Phys. Rev. Lett.},
  volume={97},
  issue={17},
  number={170409},
  year={2006},
  publisher={APS}
}

@article{colbeck2012free,
  title={Free randomness can be amplified},
  author={Colbeck, Roger and Renner, Renato},
  journal={Nature Physics},
  volume={8},
  number={6},
  pages={450--453},
  year={2012},
  publisher={Nature Research}
}

@article{hoban2011non, 
  title={Non-adaptive measurement-based quantum computation and multi-party Bell inequalities},
  author={Hoban, Matty J and Campbell, Earl T and Loukopoulos, Klearchos and Browne, Dan E},
  journal={New Journal of Physics},
  volume={13},
  issue={2},
  number={023014},
  year={2011},
  publisher={IOP Publishing}
}

@article{mukherjee2015correlations,
  title={Correlations in n-local scenario},
  author={Mukherjee, Kaushiki and Paul, Biswajit and Sarkar, Debasis},
  journal={Quantum Information Processing},
  volume={14},
  issue={6},
  pages={2025--2042},
  year={2015},
  publisher={Springer}
}

@article{tavakoli2014nonlocal,
  title={Nonlocal correlations in the star-network configuration},
  author={Tavakoli, Armin and Skrzypczyk, Paul and Cavalcanti, Daniel and Ac{\'\i}n, Antonio},
  journal={Physical Review A},
  volume={90},
  issue={6},
  number={062109},
  year={2014},
  publisher={APS}
}

@article{aolita2012fully,
  title={Fully nonlocal, monogamous, and random genuinely multipartite quantum correlations},
  author={Aolita, Leandro and Gallego, Rodrigo and Cabello, Ad{\'a}n and Ac{\'\i}n, Antonio},
  journal={Phys. Rev. Lett.},
  volume={108},
  issue={10},
  number={100401},
  year={2012},
  publisher={APS}
}   

@article{cavalcanti2010quantum,
  title={Quantum networks reveal quantum nonlocality},
  author={Cavalcanti, Daniel and Almeida, Mafalda L and Scarani, Valerio and Ac\'{i}n, Antonio},
  journal={arXiv preprint arXiv:1010.0900},
  year={2010}
}

@article{augusiak2014elemental,
  title={Elemental and tight monogamy relations in nonsignaling theories},
  author={Augusiak, Remigiusz and Demianowicz, Maciej and Paw{\l}owski, M and Tura, Jordi and Ac{\'\i}n, A},
  journal={Physical Review A},
  volume={90},
  issue={5},
  number={052323},
  year={2014},
  publisher={APS}
}

@article{barrett2012unconditionally,
  title={Unconditionally secure device-independent quantum key distribution with only two devices},
  author={Barrett, Jonathan and Colbeck, Roger and Kent, Adrian},
  journal={Physical Review A},
  volume={86},
  issue={6},
  number={062326},
  year={2012},
  publisher={APS}
}

@article{colbeck2010no,
  title={No extension of quantum theory can have improved predictive power},
  author={Colbeck, Roger and Renner, Renato},
  journal={arXiv preprint arXiv:1005.5173},
  year={2010}
}

@article{colbeck2008hidden,
  title={Hidden variable models for quantum theory cannot have any local part},
  author={Colbeck, Roger and Renner, Renato},
  journal={Phys. Rev. Lett.},
  volume={101},
  issue={5},
  number={050403},
  year={2008},
  publisher={APS}
}

@article{vazirani2014fully,
  title={Fully device-independent quantum key distribution},
  author={Vazirani, Umesh and Vidick, Thomas},
  journal={Phys. Rev. Lett.},
  volume={113},
  issue={14},
  number={140501},
  year={2014},
  publisher={APS}
}

@article{howard2014contextuality,
  title={Contextuality supplies the/magic/'for quantum computation},
  author={Howard, Mark and Wallman, Joel and Veitch, Victor and Emerson, Joseph},
  journal={Nature},
  volume={510},
  number={7505},
  pages={351--355},
  year={2014},
  publisher={Nature Research}
}

@article{bermejo2016contextuality,
  title={Contextuality as a resource for qubit quantum computation},
  author={Bermejo-Vega, Juan and Delfosse, Nicolas and Browne, Dan E and Okay, Cihan and Raussendorf, Robert},
  journal={arXiv preprint arXiv:1610.08529},
  year={2016}
}

@article{delfosse2015wigner,
  title={Wigner function negativity and contextuality in quantum computation on rebits},
  author={Delfosse, Nicolas and Guerin, Philippe Allard and Bian, Jacob and Raussendorf, Robert},
  journal={Physical Review X},
  volume={5},
  issue={2},
  number={021003},
  year={2015},
  publisher={APS}
}

@article{weilenmann2016non,
  title={Non-Shannon inequalities in the entropy vector approach to causal structures},
  author={Weilenmann, Mirjam and Colbeck, Roger},
  journal={arXiv preprint arXiv:1605.02078},
  year={2016}
}

@article{weilenmann2016non,
  title={Non-Shannon inequalities in the entropy vector approach to causal structures},
  author={Weilenmann, Mirjam and Colbeck, Roger},
  journal={arXiv preprint arXiv:1605.02078},
  year={2016}
}

@article{chaves2015device,
  title={Device-Independent Tests of Entropy},
  author={Chaves, Rafael and Brask, Jonatan Bohr and Brunner, Nicolas},
  journal={Phys. Rev. Lett.},
  volume={115},
  issue={11},
  number={110501},
  year={2015},
  publisher={APS}
}

@article{chaves2016polynomial,
  title={Polynomial bell inequalities},
  author={Chaves, Rafael},
  journal={Phys. Rev. Lett.},
  volume={116},
  issue={1},
  number={010402},
  year={2016},
  publisher={APS}
}

@article{rosset2016nonlinear,
  title={Nonlinear Bell inequalities tailored for quantum networks},
  author={Rosset, Denis and Branciard, Cyril and Barnea, Tomer Jack and P{\"u}tz, Gilles and Brunner, Nicolas and Gisin, Nicolas},
  journal={Phys. Rev. Lett.},
  volume={116},
  issue={1},
  number={010403},
  year={2016},
  publisher={APS}
}

@article{wolfe2016inflation,
  title={The Inflation Technique for Causal Inference with Latent Variables},
  author={Wolfe, Elie and Spekkens, Robert W and Fritz, Tobias},
  journal={arXiv preprint arXiv:1609.00672},
  year={2016}
}

@article{tavakoli2016bell,  
  title={Bell-type inequalities for arbitrary noncyclic networks},
  author={Tavakoli, Armin},
  journal={Physical Review A},
  volume={93},
  issue={3},
  number={030101},
  year={2016},
  publisher={APS}
}

@article{allen2016quantum,
  title={Quantum common causes and quantum causal models},
  author={Allen, John-Mark A and Barrett, Jonathan and Horsman, Dominic C and Lee, Ciaran M and Spekkens, Robert W},
  journal={arXiv preprint arXiv:1609.09487},
  year={2016}
}

@article{andreoli2017maximal,
  title={Maximal violation of n-locality inequalities in a star-shaped quantum network},
  author={Andreoli, Francesco and Carvacho, Gonzalo and Santodonato, Luca and Chaves, Rafael and Sciarrino, Fabio},
  journal={arXiv preprint arXiv:1702.08316},
  year={2017}
}

@article{tavakoli2017correlations,
  title={Correlations in star networks: from Bell inequalities to network inequalities},
  author={Tavakoli, Armin and Renou, Marc Olivier and Gisin, Nicolas and Brunner, Nicolas},
  journal={arXiv preprint arXiv:1702.03866},
  year={2017}
}

@article{lee2015causal,
  title={Causal Inference via Algebraic Geometry: Feasibility Tests for Functional Causal Structures with Two Binary Observed Variables},
  author={Lee, Ciar{\'a}n M and Spekkens, Robert W},
  journal={Journal of Causal Inference (DOI: 10.1515/jci-2016-0013), arXiv preprint arXiv:1506.03880},
  year={2017}
}

@article{saunders2017experimental,
  title={Experimental demonstration of nonbilocal quantum correlations},
  author={Saunders, Dylan J and Bennet, Adam J and Branciard, Cyril and Pryde, Geoff J},
  journal={Science Advances},
  volume={3},
  issue={4},
  number={e1602743},
  year={2017},
  publisher={American Association for the Advancement of Science}
}

@article{carvacho2017experimental,
  title={Experimental violation of local causality in a quantum network},
  author={Carvacho, Gonzalo and Andreoli, Francesco and Santodonato, Luca and Bentivegna, Marco and Chaves, Rafael and Sciarrino, Fabio},
  journal={Nature Communications},
  volume={8},
  year={2017},
  publisher={Nature Publishing Group}
}

@article{branciard2012bilocal,
  title={Bilocal versus nonbilocal correlations in entanglement-swapping experiments},
  author={Branciard, Cyril and Rosset, Denis and Gisin, Nicolas and Pironio, Stefano},
  journal={Physical Review A},
  volume={85},
  number={3},
  pages={032119},
  year={2012},
  publisher={APS}
}

@article{gisin2017allentangled,
  title={All entangled pure quantum states violate the bilocality inequality},
  author={Gisin, Nicolas and Mei, Quanxin and Tavakoli, Armin and Renou, Marc Olivier and Brunner, Nicolas},
  journal={ arXiv preprint arXiv:1702.00333},
  year={2017}
}

@article{branciard2010characterizing, 
  title={Characterizing the nonlocal correlations created via entanglement swapping},
  author={Branciard, Cyril and Gisin, Nicolas and Pironio, Stefano},
  journal={Phys. Rev. Lett.},
  volume={104},
  issue={17},
  number={170401},
  year={2010},
  publisher={APS}
}

@article{brunner2014bell,
  title={Bell nonlocality},
  author={Brunner, Nicolas and Cavalcanti, Daniel and Pironio, Stefano and Scarani, Valerio and Wehner, Stephanie},
  journal={Reviews of Modern Physics},
  volume={86},
  issue={2},
  number={419},
  year={2014},
  publisher={APS}
}

@article{acin2007device,
  title={Device-independent security of quantum cryptography against collective attacks},
  author={Ac{\'\i}n, Antonio and Brunner, Nicolas and Gisin, Nicolas and Massar, Serge and Pironio, Stefano and Scarani, Valerio},
  journal={Phys. Rev. Lett.},
  volume={98},
  issue={23},
  number={230501},
  year={2007},
  publisher={APS} 
}

@article{ramanathan2016randomness,
  title={Randomness Amplification under Minimal Fundamental Assumptions on the Devices},
  author={Ramanathan, Ravishankar and Brand{\~a}o, Fernando GSL and Horodecki, Karol and Horodecki, Micha{\l} and Horodecki, Pawe{\l} and Wojew{\'o}dka, Hanna},
  journal={Phys. Rev. Lett.},
  volume={117},
  issue={23},
  number={230501},
  year={2016},
  publisher={APS}
}
